Thermal history controls the optoelectronic response of lead halide perovskites through structure and dynamics

Lead halide perovskites are promising optoelectronic materials for photovoltaics, light emission and detection. Their efficiencies in PV now approach the detailed-balance limit, leaving stability as the principal barrier. The intrinsic instabilities studied to date centre on ionic motion within a fixed, homogeneous lattice. Here we identify a further source of intrinsic structural instability, hidden in the lattice dynamics. Mapping caesium, methylammonium and formamidinium-based compositions with Cl, Br, I and mixed X-sites through all accessible phases, using single crystal X-ray and neutron diffuse scattering, machine-learning-assisted molecular dynamics, a phenomenological octahedral tilt model and hyperspectral photoluminescence, we find that nearly every composition hosts equilibrium local structural fluctuations: dynamic nanodomains of correlated octahedral tilts, a few nanometres in size, that locally break the crystallographic symmetry. Three complementary levers control them. The A-site cation sets their symmetry, shape and anisotropy, from sparse, isotropic and tetragonal in formamidinium-based compositions to dense, anisotropic and orthorhombic in nominally cubic caesium-based ones, the most locally disordered we studied. The halide controls the dynamic disorder and the phase-transition sequence. Thermal history is the third: different ramp rates drive nominally identical compositions into distinct crystallographic phases, each with its own hidden local order. In MAPbI3, the heating rate alone changes the photoluminescence quantum efficiency across the phase transition. Because these transitions lie within device operating ranges, from terrestrial thermal cycling to the extremes of space, thermal history may shape the local structure, and hence the optoelectronic response, throughout fabrication and operation, establishing it as a design variable alongside composition.

==> SIrefs.tex <==
\makeatletter
\newlabel{S-fig:APb_flower_FA_MA}{{44}{38}{}{}{}}
\newlabel{S-fig:APb_flower_FA_MA@cref}{{[figure][44][]44}{[1][38][]38}{}{}{}}
\newlabel{S-fig:Alternative_Fits}{{17}{17}{}{}{}}
\newlabel{S-fig:Alternative_Fits@cref}{{[figure][17][]17}{[1][17][]17}{}{}{}}
\newlabel{S-fig:Correlation_Lengths}{{21}{21}{}{}{}}
\newlabel{S-fig:Correlation_Lengths@cref}{{[figure][21][]21}{[1][20][]21}{}{}{}}
\newlabel{S-fig:CsPbBr3_Energy_Windows}{{34}{31}{}{}{}}
\newlabel{S-fig:CsPbBr3_Energy_Windows@cref}{{[figure][34][]34}{[1][30][]31}{}{}{}}
\newlabel{S-fig:CsPbBr3_PhenomFit_2D}{{13}{13}{}{}{}}
\newlabel{S-fig:CsPbBr3_PhenomFit_2D@cref}{{[figure][13][]13}{[1][12][]13}{}{}{}}
\newlabel{S-fig:CsPbCl3_Twinning_Combined}{{16}{16}{}{}{}}
\newlabel{S-fig:CsPbCl3_Twinning_Combined@cref}{{[figure][16][]16}{[1][15][]16}{}{}{}}
\newlabel{S-fig:FAPbBr3_Neutron}{{52}{47}{}{}{}}
\newlabel{S-fig:FAPbBr3_Neutron@cref}{{[figure][52][]52}{[1][47][]47}{}{}{}}
\newlabel{S-fig:Flower_AllPhases}{{42}{36}{}{}{}}
\newlabel{S-fig:Flower_AllPhases@cref}{{[figure][42][]42}{[1][35][]36}{}{}{}}
\newlabel{S-fig:HK15_Compositional_Series}{{27}{26}{}{}{}}
\newlabel{S-fig:HK15_Compositional_Series@cref}{{[figure][27][]27}{[1][26][]26}{}{}{}}
\newlabel{S-fig:HK15_Pure_Halides}{{24}{24}{}{}{}}
\newlabel{S-fig:HK15_Pure_Halides@cref}{{[figure][24][]24}{[1][23][]24}{}{}{}}
\newlabel{S-fig:HalideDistribution_CoolingRate}{{26}{26}{}{}{}}
\newlabel{S-fig:HalideDistribution_CoolingRate@cref}{{[figure][26][]26}{[1][25][]26}{}{}{}}
\newlabel{S-fig:MAPbBr3_P211}{{7}{9}{}{}{}}
\newlabel{S-fig:MAPbBr3_P211@cref}{{[figure][7][]7}{[1][9][]9}{}{}{}}
\newlabel{S-fig:MAPbCl3_HK15_TempSeries}{{51}{46}{}{}{}}
\newlabel{S-fig:MAPbCl3_HK15_TempSeries@cref}{{[figure][51][]51}{[1][46][]46}{}{}{}}
\newlabel{S-fig:Schematic_Case1}{{1}{3}{}{}{}}
\newlabel{S-fig:Schematic_Case1@cref}{{[figure][1][]1}{[1][2][]3}{}{}{}}
\newlabel{S-fig:Schematic_Case2}{{2}{4}{}{}{}}
\newlabel{S-fig:Schematic_Case2@cref}{{[figure][2][]2}{[1][2][]4}{}{}{}}
\newlabel{S-fig:Schematic_Case3}{{3}{5}{}{}{}}
\newlabel{S-fig:Schematic_Case3@cref}{{[figure][3][]3}{[1][3][]5}{}{}{}}
\newlabel{S-fig:Schematic_Case4}{{4}{6}{}{}{}}
\newlabel{S-fig:Schematic_Case4@cref}{{[figure][4][]4}{[1][4][]6}{}{}{}}
\newlabel{S-fig:Schematic_Case5}{{5}{7}{}{}{}}
\newlabel{S-fig:Schematic_Case5@cref}{{[figure][5][]5}{[1][5][]7}{}{}{}}
\newlabel{sup_sec:BZ_Folding}{{9}{44}{}{}{}}
\newlabel{sup_sec:BZ_Folding@cref}{{[section][9][]9}{[1][44][]44}{}{}{}}
\newlabel{sup_sec:BeamDamage_MAPbI3}{{17}{60}{}{}{}}
\newlabel{sup_sec:BeamDamage_MAPbI3@cref}{{[section][17][]17}{[1][60][]60}{}{}{}}
\newlabel{sup_sec:DSC_MAPbI3}{{13}{47}{}{}{}}
\newlabel{sup_sec:DSC_MAPbI3@cref}{{[section][13][]13}{[1][47][]47}{}{}{}}
\newlabel{sup_sec:FAPbI3_CoolingRate}{{14}{54}{}{}{}}
\newlabel{sup_sec:FAPbI3_CoolingRate@cref}{{[section][14][]14}{[1][54][]54}{}{}{}}
\newlabel{sup_sec:MAPbCl3_Curvature}{{11}{45}{}{}{}}
\newlabel{sup_sec:MAPbCl3_Curvature@cref}{{[section][11][]11}{[1][45][]45}{}{}{}}
\newlabel{sup_sec:PL_MAPbI3}{{15}{56}{}{}{}}
\newlabel{sup_sec:PL_MAPbI3@cref}{{[section][15][]15}{[1][56][]56}{}{}{}}
\newlabel{sup_sec:Schematics}{{2}{2}{}{}{}}
\newlabel{sup_sec:Schematics@cref}{{[section][2][]2}{[1][2][]2}{}{}{}}
\newlabel{sup_sec:SigmaTheta_vs_T}{{10}{44}{}{}{}}
\newlabel{sup_sec:SigmaTheta_vs_T@cref}{{[section][10][]10}{[1][44][]44}{}{}{}}
\newlabel{sup_sec:a0a0cplus_MAPbI3}{{16}{57}{}{}{}}
\newlabel{sup_sec:a0a0cplus_MAPbI3@cref}{{[section][16][]16}{[1][57][]57}{}{}{}}
\newlabel{sup_ssec:CrossMaterial_anisotropy}{{8\,f}{41}{}{}{}}
\newlabel{sup_ssec:CrossMaterial_anisotropy@cref}{{[subsection][6][8]8\,f}{[1][41][]41}{}{}{}}
\newlabel{sup_ssec:CrossMaterial_visibility}{{8\,c}{39}{}{}{}}
\newlabel{sup_ssec:CrossMaterial_visibility@cref}{{[subsection][3][8]8\,c}{[1][38][]39}{}{}{}}
\newlabel{sup_ssec:Diffuse_Model}{{5}{11}{}{}{}}
\newlabel{sup_ssec:Diffuse_Model@cref}{{[section][5][]5}{[1][11][]11}{}{}{}}
\makeatother

